Improving concave point detection to better segment overlapped objects in images

This paper presents a method that improve state-of-the-art of the concave point detection methods as a first step to segment overlapping objects on images. It is based on the analysis of the curvature of the objects contour. The method has three main steps. First, we pre-process the original image to obtain the value of the curvature on each contour point. Second, we select regions with higher curvature and we apply a recursive algorithm to refine the previous selected regions. Finally, we obtain a concave point from each region based on the analysis of the relative position of their neighbourhood We experimentally demonstrated that a better concave points detection implies a better cluster division. In order to evaluate the quality of the concave point detection algorithm, we constructed a synthetic dataset to simulate overlapping objects, providing the position of the concave points as a ground truth. As a case study, the performance of a well-known application is evaluated, such as the splitting of overlapped cells in images of peripheral blood smears samples of patients with sickle cell anaemia. We used the proposed method to detect the concave points in clusters of cells and then we separate this clusters by ellipse fitting.

==> TitlePage_CA.tex <==
\onecolumn
\begin{center}

% % % % % % % % % % % % % % % % % % % % % % % %
%     ACTUALITZA EL CONTINGUT PEL TEU CAS     %
% % % % % % % % % % % % % % % % % % % % % % % %

\vspace*{1cm}
\includegraphics[scale=1]{figures/logo.png}

\vspace*{2.2cm}
\LARGE {\textbf{T\'itol}:} \\
\vspace*{1cm}

\noindent \Large{Autor: Nom i cognoms, i signatura\\}
\vspace*{1.5cm}

\noindent \large \textbf{Memòria del Treball de Fi de Màster} \\
\vspace*{0.5cm}
\noindent {M\`aster Universitari en Sistemes Intel·ligents (MUSI)
} \\
\noindent \large {de la} \\
\noindent \large {UNIVERSITAT DE LES ILLES BALEARS} \\
\vspace*{0.5cm}
\noindent \large {Curs Acadèmic 20xx-20xx} \\
\vspace*{1cm}

\vspace*{0.75cm}
\noindent \Large DD/MM/AAAA

\vspace*{1cm}
\noindent \large{Tutor: Nom i cognoms, i signatura\\}

%Descomenta pel tutor 2
%\vspace*{0.5cm}
%\noindent \large{Tutor: Nom i cognoms, i signatura\\}

%Descomenta pel tutor 3
%\vspace*{0.5cm}
%\noindent \large{Tutor: Nom i cognoms, i signatura\\}


\end{center}
\twocolumn
\newpage

==> TitlePage_EN.tex <==
\onecolumn
\begin{center}

% % % % % % % % % % % % % % % % % % % % % % % %
%     UPDATE THE CONTENTS IN YOUR CASE        %
% % % % % % % % % % % % % % % % % % % % % % % %

\vspace*{1cm}
\includegraphics[scale=1]{figures/logo.png}

\vspace*{2.2cm}
\LARGE {\textbf{Title}:} \\
Segmenting overlapped objects in images. A study to support the diagnosis of sickle cell disease. 
\vspace*{1cm}

\noindent \Large{Author: Miquel Miró Nicolau\\}

\vspace*{1.5cm}

\noindent \large \textbf{Master's Thesis} \\
\vspace*{0.5cm}
\noindent {Master's Degree in Intelligent Systems (MUSI)
} \\
\noindent \large {at the} \\
\noindent \large {UNIVERSITAT DE LES ILLES BALEARS} \\
\vspace*{0.5cm}
\noindent \large {Academic Year 2019-2020} \\
\vspace*{1cm}

\vspace*{0.75cm}
\noindent \Large 16/07/2020

\vspace*{1cm}
\noindent \large{Supervisor: Antoni Jaume-i-Capó}


\vspace*{0.5cm}
\noindent \large{Supervisor: Gabriel Moyà Alcover}


%Uncomment for supervisor 3
%\vspace*{0.5cm}
%\noindent \large{Supervisor: Name and surname, and signature\\}


\end{center}
\twocolumn
\newpage

==> TitlePage_ES.tex <==
\onecolumn
\begin{center}

% % % % % % % % % % % % % % % % % % % % % % % %
%     ACTUALIZA EL CONTENIDO PARA TU CASO     %
% % % % % % % % % % % % % % % % % % % % % % % %

\vspace*{1cm}
\includegraphics[scale=1]{figures/logo.png}

\vspace*{2.2cm}
\LARGE {\textbf{T\'itulo}:} \\
\vspace*{1cm}

\noindent \Large{Autor: Nombre y apellidos, y firma\\}
\vspace*{1.5cm}

\noindent \large \textbf{Memoria del Trabajo de Fin de Máster} \\
\vspace*{0.5cm}
\noindent {M\'aster Universitario en Sistemas Inteligentes (MUSI)
} \\
\noindent \large {de la} \\
\noindent \large {UNIVERSITAT DE LES ILLES BALEARS} \\
\vspace*{0.5cm}
\noindent \large {Curso Académico 20xx-20xx} \\
\vspace*{1cm}

\vspace*{0.75cm}
\noindent \Large DD/MM/AAAA

\vspace*{1cm}
\noindent \large{Tutor: Nombre y apellidos, y firma\\}

%Descomenta pel tutor 2
%\vspace*{0.5cm}
%\noindent \large{Tutor: Nombre y apellidos, y firma\\}

%Descomenta pel tutor 3
%\vspace*{0.5cm}
%\noindent \large{Tutor: Nombre y apellidos, y firma\\}


\end{center}
\twocolumn
\newpage
